ReF -- Rotation Equivariant Features for Local Feature Matching

Sparse local feature matching is pivotal for many computer vision and robotics tasks. To improve their invariance to challenging appearance conditions and viewing angles, and hence their usefulness, existing learning-based methods have primarily focused on data augmentation-based training. In this work, we propose an alternative, complementary approach that centers on inducing bias in the model architecture itself to generate `rotation-specific' features using Steerable E2-CNNs, that are then group-pooled to achieve rotation-invariant local features. We demonstrate that this high performance, rotation-specific coverage from the steerable CNNs can be expanded to all rotation angles by combining it with augmentation-trained standard CNNs which have broader coverage but are often inaccurate, thus creating a state-of-the-art rotation-robust local feature matcher. We benchmark our proposed methods against existing techniques on HPatches and a newly proposed UrbanScenes3D-Air dataset for visual place recognition. Furthermore, we present a detailed analysis of the performance effects of ensembling, robust estimation, network architecture variations, and the use of rotation priors.

==> support.tex <==
# example code for plotting - see L16, L20
import numpy as np
import os
from os.path import join
from matplotlib import rcParams as mrcp
import matplotlib.pyplot as plt

methods = ["Oct14_14-47-29_none_temporal_o4096_l1_0_ls1_split-val_resume-Oct07_00-00-40_none_temporal_o4096_l1_nord_sw_l1w1.npz", 
                   "Oct14_14-47-50_none_single_oNone_l1_0_ls1_split-val_resume-.npz",
                   "Oct14_14-48-23_none_avg_oNone_l5_0_ls1_split-val_resume-.npz",
                   "Oct14_14-48-59_none_delta_oNone_l5_0_ls1_split-val_resume-.npz",
                   "Oct14_14-50-32_none_temporal_o4096_l5_0_ls1_split-val_resume-Oct01_00-26-03_none_temporal_o4096_l10_nord_sw.npz"]

path = "/media/localuser/big2/code_outputs/seqDesc/results/20201014_nord/"

mrcp.update({'font.size': 14})

names = ['S_1', 'Raw Single Image', 'Smoothing', 'Delta', 'S_5']
for i,d in enumerate(methods):
    plt.figure(figsize=(6,4))
    pFull = join(path,d)
    dat_l1w1 = np.load(pFull)
    dbEmb = dat_l1w1['dbEmb']
    plt.scatter(dbEmb[:,0], dbEmb[:,1], c=np.arange(1000))
#     plt.title(names[i])
    plt.colorbar()
    plt.tight_layout()
#     plt.axis('off')
    plt.xticks([], [])
    plt.yticks([], [])

#     plt.savefig("images/tsne_{}.png".format(names[i]),bbox_inches='tight')
    plt.show()
